Abstract Neural Networks

Deep Neural Networks (DNNs) are rapidly being applied to safety-critical domains such as drone and airplane control, motivating techniques for verifying the safety of their behavior. Unfortunately, DNN verification is NP-hard, with current algorithms slowing exponentially with the number of nodes in the DNN. This paper introduces the notion of Abstract Neural Networks (ANNs), which can be used to soundly overapproximate DNNs while using fewer nodes. An ANN is like a DNN except weight matrices are replaced by values in a given abstract domain. We present a framework parameterized by the abstract domain and activation functions used in the DNN that can be used to construct a corresponding ANN. We present necessary and sufficient conditions on the DNN activation functions for the constructed ANN to soundly over-approximate the given DNN. Prior work on DNN abstraction was restricted to the interval domain and ReLU activation function. Our framework can be instantiated with other abstract domains such as octagons and polyhedra, as well as other activation functions such as Leaky ReLU, Sigmoid, and Hyperbolic Tangent.

==> shift_example.tex <==
We will demonstrate the use of this theorem on the LeakyReLU example from
above. Recall the original DNN is given by
\[
    f(x_1) =
    \begin{bmatrix}
        1 & 1 \\
        1 & 0 \\
        0 & 1
    \end{bmatrix}
    \mathrm{LReLU}\left(
        \begin{bmatrix}
            1 \\
            -1
        \end{bmatrix}
        \begin{bmatrix}
            x_1
        \end{bmatrix};
        0.5
    \right),
\]
and suppose we are only interested in the behavior of $f$ for $x_1 \in [-1,
1]$. Well, in that range, the output of the LReLU is \emph{at least} $-0.5$,
hence we can take $c = -0.5$. Applying the construction from the theorem, we
have
\[
    \begin{aligned}
        f'(x_1)
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \left(
        \mathrm{LReLU}'\left(
            \begin{bmatrix}
                1 \\
                -1
            \end{bmatrix}
            \begin{bmatrix}
                x_1
            \end{bmatrix};
            0.5
        \right)
        - \begin{bmatrix} 0.5 \\ 0.5 \end{bmatrix}
        \right)\\
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \mathrm{LReLU}'\left(
            \begin{bmatrix}
                1 \\
                -1
            \end{bmatrix}
            \begin{bmatrix}
                x_1
            \end{bmatrix};
            0.5
        \right)
        + \begin{bmatrix} -1 \\ -0.5 \\ -0.5 \end{bmatrix}
    \end{aligned}
\]
where
\[
    \mathrm{LReLU}'(x) \coloneqq \mathrm{max}(\mathrm{LReLU}(x) + 0.5, 0).
\]

Now consider, for example, $x_1 = -1$. In the original network we had
\[
    \begin{aligned}
        f(-1)
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \mathrm{LReLU}\left(
            \begin{bmatrix}
                1 \\
                -1
            \end{bmatrix}
            \begin{bmatrix}
                -1
            \end{bmatrix};
            0.5
        \right) \\
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \mathrm{LReLU}\left(
            \begin{bmatrix}
                -1 \\
                1
            \end{bmatrix};
            0.5
        \right) \\
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \begin{bmatrix}
            -0.5 \\
            1
        \end{bmatrix} &&(\ast) \\
        &=
        \begin{bmatrix}
            0.5 \\
            -0.5 \\
            1
        \end{bmatrix},
    \end{aligned}
\]
noticing on line $(\ast)$ that the LReLU had a negative output which caused
unsoundness. In the new network, on the other hand, we have
\[
    \begin{aligned}
        f'(-1)
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \mathrm{LReLU}'\left(
            \begin{bmatrix}
                1 \\
                -1
            \end{bmatrix}
            \begin{bmatrix}
                -1
            \end{bmatrix};
            0.5
        \right)
        + \begin{bmatrix} -1 \\ -0.5 \\ -0.5 \end{bmatrix} \\
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \mathrm{LReLU}'\left(
            \begin{bmatrix}
                -1 \\
                1
            \end{bmatrix}
            0.5
        \right)
        + \begin{bmatrix} -1 \\ -0.5 \\ -0.5 \end{bmatrix} \\
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \begin{bmatrix}
            -0.5 + 0.5 \\
            1 + 0.5
        \end{bmatrix}
        + \begin{bmatrix} -1 \\ -0.5 \\ -0.5 \end{bmatrix} \\
        &=
        \begin{bmatrix}
            1 & 1 \\
            1 & 0 \\
            0 & 1
        \end{bmatrix}
        \begin{bmatrix}
            0 \\
            1.5
        \end{bmatrix}
        + \begin{bmatrix} -1 \\ -0.5 \\ -0.5 \end{bmatrix} &&(\ast) \\
        &=
        \begin{bmatrix}
            1.5 \\
            0 \\
            1.5
        \end{bmatrix}
        + \begin{bmatrix} -1 \\ -0.5 \\ -0.5 \end{bmatrix} \\
        &=
        \begin{bmatrix}
            0.5 \\
            -0.5 \\
            1
        \end{bmatrix} \\
        &= f(1),
    \end{aligned}
\]
where on the corresponding line $(\ast)$ we can see that the activation is
non-negative.

